From Mapping to Composing: A Two-Stage Framework for Zero-shot Composed Image Retrieval

Composed Image Retrieval (CIR) is a challenging multimodal task that retrieves a target image based on a reference image and accompanying modification text. Due to the high cost of annotating CIR triplet datasets, zero-shot (ZS) CIR has gained traction as a promising alternative. Existing studies mainly focus on projection-based methods, which map an image to a single pseudo-word token. However, these methods face three critical challenges: (1) insufficient pseudo-word token representation capacity, (2) discrepancies between training and inference phases, and (3) reliance on large-scale synthetic data. To address these issues, we propose a two-stage framework where the training is accomplished from mapping to composing. In the first stage, we enhance image-to-pseudo-word token learning by introducing a visual semantic injection module and a soft text alignment objective, enabling the token to capture richer and fine-grained image information. In the second stage, we optimize the text encoder using a small amount of synthetic triplet data, enabling it to effectively extract compositional semantics by combining pseudo-word tokens with modification text for accurate target image retrieval. The strong visual-to-pseudo mapping established in the first stage provides a solid foundation for the second stage, making our approach compatible with both high- and low-quality synthetic data, and capable of achieving significant performance gains with only a small amount of synthetic data. Extensive experiments were conducted on three public datasets, achieving superior performance compared to existing approaches.

==> algorithm.tex <==


\begin{algorithm}[tb]
	\renewcommand{\algorithmicrequire}{\textbf{Input:}}
	\renewcommand{\algorithmicensure}{\textbf{Output:}}
	\caption{Confidence Estimation Algorithm}
	\label{alg:1}
	\begin{algorithmic}[1]
		\REQUIRE Noisy training dataset $\mathcal{D} = \{(V_i, S_i, T_i) \}^N_{i=1}$, max epochs $T_{max}$, iteration $I_{max}$, maximum iteration number of Sinkhorn algorithm $max\_iter$
		\ENSURE $w$ is the optimal estimated confidence of each $(V_i, S_i, T_i)$ pair.
		\FOR{$t=0,1,...,T_{max}$}  
    		\STATE Shuffle training set
    		\FOR{$n=1, ... , I_{max}$}
    		    \STATE Fetch mini-batch $\overline{\mathcal{D}}$ from $\mathcal{D}$
    		    \STATE Calculate transportation cost matrices $E_m$ and $E_l$ from two views using Eq.(8)
			    \STATE Calculate dual-view transportation costs $E$ using Eq.(9) with dual-view curriculum learning
			    \STATE Initialize $\mu^{(0)}, v^{(0)}$ as one.
		    	\WHILE{$k < max\_iter$}
			    \STATE Calculate $\mu^{(k+1)}, v^{(k+1)}$ using Eq.(6)
			    \ENDWHILE
			    \STATE Calculate optimal estimation confidence $P^{*}$ using Eq.(12)
% 			\STATE Calculate$w=diag(P^{E*})$
    		\ENDFOR
    		\STATE $w = diag(P^*)$
		\ENDFOR
	    \RETURN $w$

	\end{algorithmic}  
\end{algorithm}


==> table/ablation_param.tex <==
\begin{table} [htb!]
% \samll
% \renewcommand{\thetable}{7}
% \renewcommand{\arraystretch}{1}
% \setlength{\abovecaptionskip}{1mm} 
% \setlength{\belowcaptionskip}{-0.13cm}
% \vspace{-2em} 
\caption{The comparison of trainable parameters in methods based on mapping learning.}
\label{tab:param}
\centering 
\scalebox{1.0}{
\begin{tabular}{lcc}
\toprule
\textbf{Method} & {Learnable parameters(M)} \\
\hline
Pic2Word \cite{saito2023pic2word} &{1.64} \\
LinCIR \cite{gu2024language} &{14.16} \\
KEDs \cite{suo2024knowledge}  &{10.50} \\
ContextI2W \cite{tang2024context} &{68.47} \\
FTI4CIR \cite{lin2024fine} &{76.61} \\
\hline
Ours &{22.45}  \\
\bottomrule
\end{tabular}
 }% end of scalebox
\end{table}
\vspace{-0.9em} 
